Challenges in Mobile Multi-Device Ecosystems

Coordinated multi-display environments from the desktop, second-screen to gigapixel display walls are increasingly common. Personal and intimate mobile and wearable devices such as head-mounted displays, smartwatches, smartphones and tablets are rarely part of such multi-device ecosystems. With this paper, we contribute to a better understanding about factors that impede the creation and use of such mobile multi-device ecosystems. We base our findings on literature research and an expert survey. Specifically, we present grounded challenges relevant for the design, development and use of mobile multi-device environments.

==> oldsp.tex <==

\section{Introduction}
Multi-display systems have emerged as a mainstay for knowledge work (eg. programming or financial trading) and complex tasks (eg. city or factory management)~\cite{Terrenghi:2009}. Social applications such as gaming and second screen experiences are further extending the proliferation of increasingly complex display ecosystems. Today, we see the emergence of another range of more mobile and intimate display technology, from wrist-worn smartwatches and health devices (eg. fitbit or Microsoft Band as shown in Figure~\ref{fig:band-iphone}) to head-mounted displays~\cite{grubert2015multifi} (see Figures~\ref{fig:google-glass} and~\ref{fig:hololens}) or personal devices such as smartphones and tablets. A motivating question for us here is, can these disparate forms of displays be coupled and coordinated to realise ``proximate display environments'', with on and around the body interaction as shown in Figure~\ref{fig:multifi} from ~\cite{grubert2015multifi}?   

Of course, once we start to use an ecosystem of connected and coupled personal or appropriated displays (as shown in Figure~\ref{fig:band-iphone}), a number of challenges arise. How will we manage our attention, visual focus or awareness as our interaction is being spread across an ever wider display ecosystem? Which of our elements of human perception  will this challenge? And will this form of interaction raise serious social challenges for us to face? These are the issues we seek to begin to address in this paper as distinct from the design and technology issues~\cite{quig-per-soc-mobilehci} introduced elsewhere. 

%When we consider the use of wearable multi-display systems in the world, there are a number of social challenges this presents, including; privacy, social acceptability, social participation, social exclusion, social engagement and social disorganization.

%some of these devices expect to operate in isolation, affording the user and ``island of interaction'', all too often locking their data into a silo. However, we are now seeing more of these devices being designed to work in device ecosystems, i.e. in conjunction with additional personal displays with complementary device characteristics. Take, for example, smartwatches notifying their users about an incoming e-mail on their wrist but deferring the reading and writing of mails to an associated smartphone. Other devices can be appropriated to work in conjunction with additional displays. For example, a smartphone and a tablet can be used to distribute tasks across those devices (e.g., displaying a contact list on the mobile phone and an associated text document on the tablet). Many more permutations involving personal to public or appropriated to intimate displays are possible~\cite{Terrenghi:2009}.  

%However, to date, what is not well understood is which factors inhibit or support the interaction across multiple displays on and around the body ie. ``Body Proximate''. Within this paper we review four key design and technological challenges inherent in body proximate display ecosystems. 

\section{Perceptual Challenges}
%Human perception involves a combination of factors, including our low level sensory inputs, processing these inputs into intermediate information, combination of this with each person's existing knowledge and our implicit and explicit attention. Each of these factors has limitations, from the physiological to the cognitive, which presents us with a series of perceptual challenges and opportunities in the research, design and development of wearable multi-display interaction.

There are numerous challenges with human perception in body proximate display ecosystems from physiological to cognitive levels. Such issues stem from varying display resolutions, luminance, effective visual fidelities, visual interference, color or contrast in display overlap which can be experienced with body proximate ecosystems. Here we focus on the issues of display switching, focus (or accomodation) and field of view. 


\paragraph{Display Switching} Existing research has identified the cost of display switching~\cite{Rashid:Nacenta:Quigley:2012} and the factors which influence visual attention in multi-display user interfaces~\cite{Rashid:2012:CDS:2254556.2254577}. These factors include display contiguity (as shown in Figure~\ref{fig:contiguity}), angular coverage, content coordination, input directness and input-display correspondence. Further physiological issues arise with depth discontiguous displays, field of view, visual acuity or indeed blind spots with monocular displays employed in multi-display interaction.

%In human vision the ciliary muscles change the shape of the lens in our eyes so we can focus (fixate) on objects at different distances. 

%The Iris controls how much light is let in through the pupil of your eye, so that in low light conditions the pupil expands while in bright conditions it contracts. These factors alter how light from the environment and hence our multi-display environments reaches the retina of our eyes.

\paragraph{Focus in Human Vision} The shape of our lens and iris alters how much light enters and how our eyes focus. However, our eyes cannot focus sharply on two displays which are near and far simultaneously. If the virtual display plane of an optical see-through head-mounted device is in sharp focus, then effectively closer or distant displays won't be. This can be easily seen with a smartwatch which is in focus but is then surrounded by unfocused input from displays effectively further from the eye. The effective distance, not actual distance, needs to be considered as devices, such as optical see-through displays (eg. Google Glass) often employ optical techniques to generate images at distances which are easier for the eye to accomodate. A further issue to consider is that as the ciliary muscles in our eyes age, our range of accommodation declines. As a result, with body proximate ecosystems we can experience a mixed focus interface with some elements in sharp focus while others are defocused. This is quite unlike typical display environments, where each element of the display is typically in focus.
 %Multi-display environments embedded in the physical environment can exploit the fact that the eye needs no time with depth contiguous displays or little time to accommodate for small effective changes in the discontinuous nature of the display space.
 
Another byproduct of our eyes inability to focus sharply on two distances, is that it then takes time for the eye to refocus on objects at different distances. In addition, the speed of this process also declines as the muscles age.  However, with body proximate ecosystems the eye will need noticeable amounts of time (eg. 300~msec latency and 1000~msec stabilisation period~\cite{charman-2008}) for the focal power of the eye to adapt in markedly discontiguous display spaces. Further, these accomodation times don't include movements if the displays are ``visually field discontiguous''~\cite{Rashid:Nacenta:Quigley:2012}.

\paragraph{Field of View} Humans have a limited field of view and an age diminished ``useful field of view'' (UFOV)~\cite{Richards-2006}, which needs to be considered. Excluding head rotation, the typical field of view for a human has a difference between the horizontal and vertical field of view, an area of binocular overlap and areas of monocular far peripheral vision. "For many of our interaction tasks the UFOV varies between younger and older people. A 36 degree field of view will be practical in many situations ~\cite{Richards-2006}. Within each person's field of view we can also distinguish regions of central (ie. foveal, central, paracentral and macular) and peripheral (near, mid and far) vision. The useful field of view above, typically includes both central and largely near peripheral parts of vision.

\section{Conclusion}
Within this paper we have considered some of the social  and perceptual challenges and questions raised in interaction with multiple displays on and around the body, including smartwatches, smartglasses and smartphones. Body proximate display applications give rise to a range of other issues which challenge the limits of the human being and our social sphere at varying scales (see Figure ~\ref{fig:taxonomy}). The social challenges may simply be opportunities while adapting our display environments to accommodate for our field of view, current focus and the cost of display switching are just some of the perceptual challenges we face. Through discussing these challenges and questions we hope to contribute to shaping the research agenda of interaction with multi-display environments \emph{on and around the body} ie. body proximate display ecosystems.



\section{Social Challenges}
Beyond our personal perception of the world, there are a number of social challenges that body proximate ecosystems systems present, including privacy, social acceptability, social participation, social exclusion and social engagement. 


\paragraph{Privacy} presents a major challenge in the use of public or semi-public displays as part of a wearable multi-display ecosystem. We can consider such forms of social interaction with technology at different scales from inch to chain and beyond~\cite{Terrenghi:2009} as shown in Figure~\ref{fig:taxonomy}. Personal devices overcome the privacy challenge by use of private environments, use at an intimate distance, privacy screens or non-visual modalities. Questions arise when we consider how we might share content on intimate displays, at varying scales, different social interaction types or even share content spanning multiple private displays.

\begin{figure}
\includegraphics[width=0.9\columnwidth]{figures/social-interaction-scale.png}
    \centering

\caption{Multi-person-display ecosystem taxonomy~\cite{Terrenghi:2009}, social interaction support and ecosystem scale}\label{fig:taxonomy}
\end{figure}


\paragraph{Social acceptability} The use of wearable on body displays presents a range of social acceptability issues. Some of the inherent form factors (eg. Microsoft Hololens in Figure~\ref{fig:hololens}) can present acceptability challenges. In addition, existing research has explored the suitability of different parts of the body for gestural inputs, along with issues of social norms and behaviour~\cite{Profita:2013:DMM:2493988.2494331}. Here, body proximate displays introduce new challenges as the coordination and movement of multiple displays can require unusual inter-display coordination and body orientation. Also, in contrast to touch-only operated displays such as smartphones, the manipulations of multiple body proximate displays through spatial gestures are more visible whereas the effects of those actions remain hidden to bystanders~\cite{reeves2005designing}. Depending on the social situation this could lead to inhibited or non-use of an interactive system, similar to observations made for handheld Augmented Reality systems \cite{grubert2012playing, grubert2013playing}. Further issues arise from the use of shared or public display elements within an ecosystem.  All of these issues are modulated by difference cultures, work practices, age, familiarity with technology an evolving social norms for new technology behaviours.   

\paragraph{Social participation} Today, civic discourse is impacted by the isolation that technologies provide people. For example, the ``filter bubble~\cite{Pariser:2011:FBI:2029079}'' stems from the personalisation in search results presented to individual people. Such bubbles can socially isolate people from one another, into their own economic, political, cultural and hence ideological groups. With body proximate ecosystems, we might further encourage people into ``interaction bubbles'' which isolates them further from others and discourages interpersonal interaction. The ``in-your-face nature'' of what is proposed, is unlike other forms of technology. 

\paragraph{Social exclusion} Mirroring the problems in social participation are the further challenges of social exclusion. By augmenting our interactions with body proximate ecosystems we are changing the nature of our interaction with the world. Many personal technologies reside out of sight, whereas wearable and on body displays present a visible digital alienation to those without access to such technology. By allowing some to see and experience more than others can see are we further disenfranchising people? Do these technologies further reinforce a digital social stratification we are already witnessing? 

\paragraph{Social engagement} In using semipublic or public displays as part of an egocentric body proximate ecosystem, issues of performance and social engagement present themselves. These challenges are also opportunities for improved social engagement between people but also draw into question the appropriateness of any device appropriation. Fair use, sharing space or time, along with the use of non-visual modalities present challenges for the design and deployment of such systems.    

\section{Conclusion}
Within this paper we have considered some of the social  and perceptual challenges and questions raised in interaction with multiple displays on and around the body, including smartwatches, smartglasses and smartphones. Body proximate display applications give rise to a range of other issues which challenge the limits of the human being and our social sphere at varying scales (see Figure ~\ref{fig:taxonomy}). The social challenges may simply be opportunities while adapting our display environments to accommodate for our field of view, current focus and the cost of display switching are just some of the perceptual challenges we face. Through discussing these challenges and questions we hope to contribute to shaping the research agenda of interaction with multi-display environments \emph{on and around the body} ie. body proximate display ecosystems.

==> relatedwork.tex <==
\section{relatedwork}
